BoolE: Exact Symbolic Reasoning via Boolean Equality Saturation

Boolean symbolic reasoning for gate-level netlists is a critical step in verification, logic and datapath synthesis, and hardware security. Specifically, reasoning datapath and adder tree in bit-blasted Boolean networks is particularly crucial for verification and synthesis, and challenging. Conventional approaches either fail to accurately (exactly) identify the function blocks of the designs in gate-level netlist with structural hashing and symbolic propagation, or their reasoning performance is highly sensitive to structure modifications caused by technology mapping or logic optimization. This paper introduces BoolE, an exact symbolic reasoning framework for Boolean netlists using equality saturation. BoolE optimizes scalability and performance by integrating domain-specific Boolean ruleset for term rewriting. We incorporate a novel extraction algorithm into BoolE to enhance its structural insight and computational efficiency, which adeptly identifies and captures multi-input, multi-output high-level structures (e.g., full adder) in the reconstructed e-graph. Our experiments show that BoolE surpasses state-of-the-art symbolic reasoning baselines, including the conventional functional approach (ABC) and machine learning-based method (Gamora). Specifically, we evaluated its performance on various multiplier architecture with different configurations. Our results show that BoolE identifies $3.53\times$ and $3.01\times$ more exact full adders than ABC in carry-save array and Booth-encoded multipliers, respectively. Additionally, we integrated BoolE into multiplier formal verification tasks, where it significantly accelerates the performance of traditional formal verification tools using computer algebra, demonstrated over four orders of magnitude runtime improvements.

==> bib.tex <==
\begin{thebibliography}{00}
\bibitem{Bengio+chapter2007}Bengio, Y. \& LeCun, Y. Scaling Learning Algorithms Towards AI. {\em Large Scale Kernel Machines}. (2007)
\bibitem{zhou2021rethinking}Zhou, Y., Dong, X., Akin, B., Tan, M., Peng, D., Meng, T., Yazdanbakhsh, A., Huang, D., Narayanaswami, R. \& Laudon, J. Rethinking co-design of neural architectures and hardware accelerators. {\em ArXiv Preprint ArXiv:2102.08619}. (2021)
\bibitem{chen2018tvm}Chen, T., Moreau, T., Jiang, Z., Zheng, L., Yan, E., Shen, H., Cowan, M., Wang, L., Hu, Y., Ceze, L. \& Others {TVM}: An automated end-to-end optimizing compiler for deep learning. {\em 13th {USENIX} Symposium On Operating Systems Design And Implementation ({OSDI} 18)}. pp. 578-594 (2018)
\bibitem{Hinton06}Hinton, G., Osindero, S. \& Teh, Y. A Fast Learning Algorithm for Deep Belief Nets. {\em Neural Computation}. \textbf{18} pp. 1527-1554 (2006)
\bibitem{goodfellow2016deep}Goodfellow, I., Bengio, Y., Courville, A. \& Bengio, Y. Deep learning. (MIT Press,2016)
\bibitem{hochreiter1997long}Hochreiter, S. \& Schmidhuber, J. Long short-term memory. {\em Neural Computation}. \textbf{9}, 1735-1780 (1997)
\bibitem{boroumand2021mitigating}Boroumand, A., Ghose, S., Akin, B., Narayanaswami, R., Oliveira, G., Ma, X., Shiu, E. \& Mutlu, O. Mitigating Edge Machine Learning Inference Bottlenecks: An Empirical Study on Accelerating Google Edge Models. {\em ArXiv Preprint ArXiv:2103.00768}. (2021)
\bibitem{yazdanbakhsh2021evaluation}Yazdanbakhsh, A., Seshadri, K., Akin, B., Laudon, J. \& Narayanaswami, R. An evaluation of edge tpu accelerators for convolutional neural networks. {\em ArXiv Preprint ArXiv:2102.10423}. (2021)
\bibitem{jouppi2017datacenter}Jouppi, N., Young, C., Patil, N., Patterson, D., Agrawal, G., Bajwa, R., Bates, S., Bhatia, S., Boden, N., Borchers, A. \& Others In-datacenter performance analysis of a tensor processing unit. {\em Proceedings Of The 44th Annual International Symposium On Computer Architecture}. pp. 1-12 (2017)
\bibitem{sheng2021deep}Sheng, S., Chen, P., Chen, Z., Wu, L. \& Yao, Y. Deep Reinforcement Learning-Based Task Scheduling in IoT Edge Computing. {\em Sensors}. \textbf{21}, 1666 (2021)
\bibitem{chen2019deep}Chen, H. \& Shen, M. A Deep-Reinforcement-Learning-Based Scheduler for FPGA HLS. {\em 2019 IEEE/ACM International Conference On Computer-Aided Design (ICCAD)}. pp. 1-8 (2019)
\bibitem{vaswani2017attention}Vaswani, A., Shazeer, N., Parmar, N., Uszkoreit, J., Jones, L., Gomez, A., Kaiser, Ł. \& Polosukhin, I. Attention is all you need. {\em Advances In Neural Information Processing Systems}. pp. 5998-6008 (2017)
\bibitem{williams1992simple}Williams, R. Simple statistical gradient-following algorithms for connectionist reinforcement learning. {\em Machine Learning}. \textbf{8}, 229-256 (1992)
\bibitem{bello2016neural}Bello, I., Pham, H., Le, Q., Norouzi, M. \& Bengio, S. Neural combinatorial optimization with reinforcement learning. {\em ArXiv Preprint ArXiv:1611.09940}. (2016)
\bibitem{chollet2017xception}Chollet, F. Xception: Deep learning with depthwise separable convolutions. {\em Proceedings Of The IEEE Conference On Computer Vision And Pattern Recognition}. pp. 1251-1258 (2017)
\bibitem{he2016identity}He, K., Zhang, X., Ren, S. \& Sun, J. Identity mappings in deep residual networks. {\em European Conference On Computer Vision}. pp. 630-645 (2016)
\bibitem{szegedy2017inception}Szegedy, C., Ioffe, S., Vanhoucke, V. \& Alemi, A. Inception-v4, inception-resnet and the impact of residual connections on learning. {\em Thirty-first AAAI Conference On Artificial Intelligence}. (2017)
\bibitem{he2016deep}He, K., Zhang, X., Ren, S. \& Sun, J. Deep residual learning for image recognition. {\em Proceedings Of The IEEE Conference On Computer Vision And Pattern Recognition}. pp. 770-778 (2016)
\bibitem{huang2017densely}Huang, G., Liu, Z., Van Der Maaten, L. \& Weinberger, K. Densely connected convolutional networks. {\em Proceedings Of The IEEE Conference On Computer Vision And Pattern Recognition}. pp. 4700-4708 (2017)
\bibitem{sanders2010cuda}Sanders, J. \& Kandrot, E. CUDA by example: an introduction to general-purpose GPU programming. (Addison-Wesley Professional,2010)
\bibitem{yu2018semantic}Yu, B., Yang, L. \& Chen, F. Semantic segmentation for high spatial resolution remote sensing images based on convolution neural network and pyramid pooling module. {\em IEEE Journal Of Selected Topics In Applied Earth Observations And Remote Sensing}. \textbf{11}, 3252-3261 (2018)
\bibitem{abadi2016tensorflow}Abadi, M., Barham, P., Chen, J., Chen, Z., Davis, A., Dean, J., Devin, M., Ghemawat, S., Irving, G., Isard, M. \& Others Tensorflow: A system for large-scale machine learning. {\em 12th {USENIX} Symposium On Operating Systems Design And Implementation ({OSDI} 16)}. pp. 265-283 (2016)
\bibitem{kuchcinski2003constraints}Kuchcinski, K. Constraints-driven scheduling and resource assignment. {\em ACM Transactions On Design Automation Of Electronic Systems (TODAES)}. \textbf{8}, 355-383 (2003)
\bibitem{lente2014exponential}Lenté, C., Liedloff, M., Soukhal, A. \& T'Kindt, V. Exponential algorithms for scheduling problems.  (2014)
\bibitem{mao2019learning}Mao, H., Schwarzkopf, M., Venkatakrishnan, S., Meng, Z. \& Alizadeh, M. Learning scheduling algorithms for data processing clusters. {\em Proceedings Of The ACM Special Interest Group On Data Communication}. pp. 270-288 (2019)
\bibitem{goyal2017accurate}Goyal, P., Dollár, P., Girshick, R., Noordhuis, P., Wesolowski, L., Kyrola, A., Tulloch, A., Jia, Y. \& He, K. Accurate, large minibatch sgd: Training imagenet in 1 hour. {\em ArXiv Preprint ArXiv:1706.02677}. (2017)
\bibitem{smith2017bayesian}Smith, S. \& Le, Q. A bayesian perspective on generalization and stochastic gradient descent. {\em ArXiv Preprint ArXiv:1710.06451}. (2017)
\bibitem{keskar2016large}Keskar, N., Mudigere, D., Nocedal, J., Smelyanskiy, M. \& Tang, P. On large-batch training for deep learning: Generalization gap and sharp minima. {\em ArXiv Preprint ArXiv:1609.04836}. (2016)
\bibitem{welling2011bayesian}Welling, M. \& Teh, Y. Bayesian learning via stochastic gradient Langevin dynamics. {\em Proceedings Of The 28th International Conference On Machine Learning (ICML-11)}. pp. 681-688 (2011)
\bibitem{zagoruyko2016wide}Zagoruyko, S. \& Komodakis, N. Wide residual networks. {\em ArXiv Preprint ArXiv:1605.07146}. (2016)
\bibitem{zhao2019adaptive}Zhao, R., Vogel, B. \& Ahmed, T. Adaptive Loss Scaling for Mixed Precision Training. {\em ArXiv Preprint ArXiv:1910.12385}. (2019)
\bibitem{krizhevsky2014one}Krizhevsky, A. One weird trick for parallelizing convolutional neural networks. {\em ArXiv Preprint ArXiv:1404.5997}. (2014)
\bibitem{peng2018megdet}Peng, C., Xiao, T., Li, Z., Jiang, Y., Zhang, X., Jia, K., Yu, G. \& Sun, J. Megdet: A large mini-batch object detector. {\em Proceedings Of The IEEE Conference On Computer Vision And Pattern Recognition}. pp. 6181-6189 (2018)
\bibitem{akiba2017extremely}Akiba, T., Suzuki, S. \& Fukuda, K. Extremely large minibatch sgd: Training resnet-50 on imagenet in 15 minutes. {\em ArXiv Preprint ArXiv:1711.04325}. (2017)
\bibitem{you2019reducing}You, Y., Li, J., Hseu, J., Song, X., Demmel, J. \& Hsieh, C. Reducing BERT pre-training time from 3 days to 76 minutes. {\em ArXiv Preprint ArXiv:1904.00962}. (2019)
\bibitem{you2017imagenet}You, Y., Zhang, Z., Demmel, J., Keutzer, K. \& Hsieh, C. Imagenet training in 24 minutes. {\em ArXiv Preprint ArXiv:1709.05011}. (2017)
\bibitem{lin2017deep}Lin, Y., Han, S., Mao, H., Wang, Y. \& Dally, W. Deep gradient compression: Reducing the communication bandwidth for distributed training. {\em ArXiv Preprint ArXiv:1712.01887}. (2017)
\bibitem{hoffer2017train}Hoffer, E., Hubara, I. \& Soudry, D. Train longer, generalize better: closing the generalization gap in large batch training of neural networks. {\em Advances In Neural Information Processing Systems}. pp. 1731-1741 (2017)
\bibitem{smith2017don}Smith, S., Kindermans, P., Ying, C. \& Le, Q. Don't decay the learning rate, increase the batch size. {\em ArXiv Preprint ArXiv:1711.00489}. (2017)
\bibitem{wu2018group}Wu, Y. \& He, K. Group normalization. {\em Proceedings Of The European Conference On Computer Vision (ECCV)}. pp. 3-19 (2018)
\bibitem{duong-etal-2015}Duong, L., Cohn, T., Bird, S. \& Cook, P. Low Resource Dependency Parsing: Cross-lingual Parameter Sharing in a Neural Network Parser. {\em Proc. Annual Meeting Of The Association For Computational Linguistics And The International Joint Conference On Natural Language Processing}. pp. 845-850 (2015,7)
\bibitem{Caruana1993}Caruana, R. Multitask Learning: A Knowledge-Based Source of Inductive Bias. {\em Proc. International Conference On Machine Learning}. pp. 41-48 (1993)
\bibitem{wang19d}Wang, Z., Zhou, Y., Liang, Y. \& Lan, G. Stochastic Variance-Reduced Cubic Regularization for Nonconvex Optimization. {\em Proc. International Conference On Artificial Intelligence And Statistics (AISTATS)}. \textbf{89} pp. 2731-2740 (2019,4)
\bibitem{zhou2018}Zhou, Y., Wang, Z. \& Liang, Y. Convergence of Cubic Regularization for Nonconvex Optimization under Kundefined Property. {\em Proc. International Conference On Neural Information Processing Systems (NeurIPS)}. pp. 3764-3773 (2018)
\bibitem{nesterov2006}Nesterov, Y. \& Polyak, B. Cubic Regularization of Newton Method and Its Global Performance. {\em Mathematical Programming}. \textbf{108}, 177-205 (2006,8)
\bibitem{Toh2010}Toh, K. \& Yun, S. An Accelerated Proximal Gradient Algorithm for Nuclear Norm Regularized Least Squares Problems. {\em Pacific Journal Of Optimization}. \textbf{6} (2010,9)
\bibitem{candes2012}Candès, E. \& Recht, B. Exact Matrix Completion via Convex Optimization. {\em Communications Of The ACM}. \textbf{55}, 111-119 (2012,6)
\bibitem{Simon2013}Simon, N., Friedman, J., Hastie, T. \& Tibshirani, R. A Sparse-Group Lasso. {\em Journal Of Computational And Graphical Statistics}. \textbf{22}, 231-245 (2013)
\bibitem{Tibshirani2011}Tibshirani, R. Regression shrinkage and selection via the lasso: a retrospective. {\em Journal Of The Royal Statistical Society: Series B (Statistical Methodology)}. \textbf{73}, 273-282 (2011)
\bibitem{Krogh1991}Krogh, A. \& Hertz, J. A Simple Weight Decay Can Improve Generalization. {\em Proc. Advances In Neural Information Processing Systems (NeurIPS)}. pp. 950-957 (1992)
\bibitem{sandler2018mobilenetv2}Sandler, M., Howard, A., Zhu, M., Zhmoginov, A. \& Chen, L. Mobilenetv2: Inverted residuals and linear bottlenecks. {\em Proceedings Of The IEEE Conference On Computer Vision And Pattern Recognition}. pp. 4510-4520 (2018)
\bibitem{simonyan2014vgg}Simonyan, K. \& Zisserman, A. Very deep convolutional networks for large-scale image recognition. {\em ArXiv Preprint ArXiv:1409.1556}. (2014)
\bibitem{krizhevsky2014cifar}Krizhevsky, A., Nair, V. \& Hinton, G. The cifar-10 dataset. {\em Online: Http://www. Cs. Toronto. Edu/kriz/cifar. Html}. \textbf{55} (2014)
\bibitem{minibatchSGD}Robbins, H. \& Monro, S. A Stochastic Approximation Method. {\em Ann. Math. Statist.}. \textbf{22}, 400-407 (1951,9), https://doi.org/10.1214/aoms/1177729586
\bibitem{fb_largebatch}Goyal, P., Dollár, P., Girshick, R., Noordhuis, P., Wesolowski, L., Kyrola, A., Tulloch, A., Jia, Y. \& He, K. Accurate, Large Minibatch SGD: Training ImageNet in 1 Hour. {\em CoRR}. \textbf{abs/1706.02677} (2017), http://arxiv.org/abs/1706.02677
\bibitem{google_largebatch}Smith, S., Kindermans, P. \& Le, Q. Don't Decay the Learning Rate, Increase the Batch Size. {\em International Conference On Learning Representations}. (2018), https://openreview.net/forum?id=B1Yy1BxCZ
\bibitem{momentumSGD}Sutskever, I., Martens, J., Dahl, G. \& Hinton, G. On the Importance of Initialization and Momentum in Deep Learning. {\em Proceedings Of The 30th International Conference On International Conference On Machine Learning - Volume 28}. pp. III-1139–III–1147 (2013)
\bibitem{largebatch1}Chen, K. \& Huo, Q. Scalable training of deep learning machines by incremental block training with intra-block parallel optimization and blockwise model-update filtering. {\em 2016 IEEE International Conference On Acoustics, Speech And Signal Processing (ICASSP)}. pp. 5880-5884 (2016)
\bibitem{largebatch2}Keskar, N., Mudigere, D., Nocedal, J., Smelyanskiy, M. \& Tang, P. On Large-Batch Training for Deep Learning: Generalization Gap and Sharp Minima. {\em CoRR}. \textbf{abs/1609.04836} (2016), http://arxiv.org/abs/1609.04836
\bibitem{largebatch3}Masters, D. \& Luschi, C. Revisiting Small Batch Training for Deep Neural Networks. {\em CoRR}. \textbf{abs/1804.07612} (2018), http://arxiv.org/abs/1804.07612
\bibitem{lars}You, Y., Gitman, I. \& Ginsburg, B. Scaling SGD Batch Size to 32K for ImageNet Training. {\em CoRR}. \textbf{abs/1708.03888} (2017), http://arxiv.org/abs/1708.03888
\bibitem{anisotropic_noise}Zhu, Z., Wu, J., Yu, B., Wu, L. \& Ma, J. The Anisotropic Noise in Stochastic Gradient Descent: Its Behavior of Escaping from Sharp Minima and Regularization Effects.  (2018)
\bibitem{grover2016node2vec}Grover, A. \& Leskovec, J. node2vec: Scalable feature learning for networks. {\em Proceedings Of The 22nd ACM SIGKDD International Conference On Knowledge Discovery And Data Mining}. pp. 855-864 (2016)
\bibitem{liao2019efficient}Liao, R., Li, Y., Song, Y., Wang, S., Hamilton, W., Duvenaud, D., Urtasun, R. \& Zemel, R. Efficient graph generation with graph recurrent attention networks. {\em Advances In Neural Information Processing Systems}. pp. 4255-4265 (2019)
\bibitem{silver2017mastering}Silver, D., Hubert, T., Schrittwieser, J., Antonoglou, I., Lai, M., Guez, A., Lanctot, M., Sifre, L., Kumaran, D., Graepel, T. \& Others Mastering chess and shogi by self-play with a general reinforcement learning algorithm. {\em ArXiv Preprint ArXiv:1712.01815}. (2017)
\bibitem{wen2019empirical}Wen, Y., Luk, K., Gazeau, M., Zhang, G., Chan, H. \& Ba, J. An Empirical Study of Large-Batch Stochastic Gradient Descent with Structured Covariance Noise.  (2019)
\bibitem{yadavwelcome}Yadav, P., Gupta, M. \& Liptak, V. Welcome Message from SenSys-ML’20 Chairs. 
\bibitem{rotem2018glow}Rotem, N., Fix, J., Abdulrasool, S., Catron, G., Deng, S., Dzhabarov, R., Gibson, N., Hegeman, J., Lele, M., Levenstein, R. \& Others Glow: Graph lowering compiler techniques for neural networks. {\em ArXiv Preprint ArXiv:1805.00907}. (2018)
\bibitem{bleiweiss2008gpu}Bleiweiss, A. GPU accelerated pathfinding. {\em Proceedings Of The 23rd ACM SIGGRAPH/EUROGRAPHICS Symposium On Graphics Hardware}. pp. 65-74 (2008)
\bibitem{gambardella1995ant}Gambardella, L. \& Dorigo, M. Ant-Q: A reinforcement learning approach to the traveling salesman problem. {\em Machine Learning Proceedings 1995}. pp. 252-260 (1995)
\bibitem{karapetyan2017markov}Karapetyan, D., Punnen, A. \& Parkes, A. Markov chain methods for the bipartite boolean quadratic programming problem. {\em European Journal Of Operational Research}. \textbf{260}, 494-506 (2017)
\bibitem{khalil2017learning}Khalil, E., Dai, H., Zhang, Y., Dilkina, B. \& Song, L. Learning combinatorial optimization algorithms over graphs. {\em Advances In Neural Information Processing Systems}. pp. 6348-6358 (2017)
\bibitem{sharafi2015conceptual}Sharafi, P., Teh, L. \& Hadi, M. Conceptual design optimization of rectilinear building frames: A knapsack problem approach. {\em Engineering Optimization}. \textbf{47}, 1303-1323 (2015)
\bibitem{lodi2017learning}Lodi, A. \& Zarpellon, G. On learning and branching: a survey. {\em Top}. \textbf{25}, 207-236 (2017)
\bibitem{chen2019learning}Chen, X. \& Tian, Y. Learning to perform local rewriting for combinatorial optimization. {\em Advances In Neural Information Processing Systems}. pp. 6281-6292 (2019)
\bibitem{nazari2018reinforcement}Nazari, M., Oroojlooy, A., Snyder, L. \& Takác, M. Reinforcement learning for solving the vehicle routing problem. {\em Advances In Neural Information Processing Systems}. pp. 9839-9849 (2018)
\bibitem{burger2020mobile}Burger, B., Maffettone, P., Gusev, V., Aitchison, C., Bai, Y., Wang, X., Li, X., Alston, B., Li, B., Clowes, R. \& Others A Mobile Robotic Chemist. {\em Nature}. \textbf{583}, 237-241 (2020)
\bibitem{martin2018middle}Martin, F., Wang, C., Petty, T., Wang, W. \& Wilkins, P. Middle school students’ social media use. {\em Journal Of Educational Technology & Society}. \textbf{21}, 213-224 (2018)
\bibitem{gleason2018digital}Gleason, B. \& Von Gillern, S. Digital citizenship with social media: Participatory practices of teaching and learning in secondary education. {\em Journal Of Educational Technology & Society}. \textbf{21}, 200-212 (2018)
\bibitem{cappart2019improving}Cappart, Q., Goutierre, E., Bergman, D. \& Rousseau, L. Improving optimization bounds using machine learning: Decision diagrams meet deep reinforcement learning. {\em Proceedings Of The AAAI Conference On Artificial Intelligence}. \textbf{33} pp. 1443-1451 (2019)
\bibitem{song2019co}Song, J., Lanka, R., Yue, Y. \& Ono, M. Co-training for policy learning. {\em ArXiv Preprint ArXiv:1907.04484}. (2019)
\bibitem{junger1995traveling}Jünger, M., Reinelt, G. \& Rinaldi, G. The traveling salesman problem. {\em Handbooks In Operations Research And Management Science}. \textbf{7} pp. 225-330 (1995)
\bibitem{he2014learning}He, H., Daume III, H. \& Eisner, J. Learning to search in branch and bound algorithms. {\em Advances In Neural Information Processing Systems}. pp. 3293-3301 (2014)
\bibitem{vinyals2015pointer}Vinyals, O., Fortunato, M. \& Jaitly, N. Pointer networks. {\em Advances In Neural Information Processing Systems}. pp. 2692-2700 (2015)
\bibitem{hamilton2017inductive}Hamilton, W., Ying, Z. \& Leskovec, J. Inductive representation learning on large graphs. {\em Advances In Neural Information Processing Systems}. pp. 1024-1034 (2017)
\bibitem{sutskever2014sequence}Sutskever, I., Vinyals, O. \& Le, Q. Sequence to sequence learning with neural networks. {\em Advances In Neural Information Processing Systems}. pp. 3104-3112 (2014)
\bibitem{silver2014deterministic}Silver, D., Lever, G., Heess, N., Degris, T., Wierstra, D. \& Riedmiller, M. Deterministic policy gradient algorithms.  (2014)
\bibitem{watkins1992q}Watkins, C. \& Dayan, P. Q-learning. {\em Machine Learning}. \textbf{8}, 279-292 (1992)
\bibitem{yu2020meta}Yu, T., Quillen, D., He, Z., Julian, R., Hausman, K., Finn, C. \& Levine, S. Meta-world: A benchmark and evaluation for multi-task and meta reinforcement learning. {\em Conference On Robot Learning}. pp. 1094-1100 (2020)
\bibitem{rakelly2019efficient}Rakelly, K., Zhou, A., Finn, C., Levine, S. \& Quillen, D. Efficient off-policy meta-reinforcement learning via probabilistic context variables. {\em International Conference On Machine Learning}. pp. 5331-5340 (2019)
\bibitem{gupta2018meta}Gupta, A., Mendonca, R., Liu, Y., Abbeel, P. \& Levine, S. Meta-reinforcement learning of structured exploration strategies. {\em Advances In Neural Information Processing Systems}. pp. 5302-5311 (2018)
\bibitem{kingma2014adam}Kingma, D. \& Ba, J. Adam: A method for stochastic optimization. {\em ArXiv Preprint ArXiv:1412.6980}. (2014)
\bibitem{ruder2016overview}Ruder, S. An overview of gradient descent optimization algorithms. {\em ArXiv Preprint ArXiv:1609.04747}. (2016)
\bibitem{wu2016google}Wu, Y., Schuster, M., Chen, Z., Le, Q., Norouzi, M., Macherey, W., Krikun, M., Cao, Y., Gao, Q., Macherey, K. \& Others Google's neural machine translation system: Bridging the gap between human and machine translation. {\em ArXiv Preprint ArXiv:1609.08144}. (2016)
\bibitem{lpddr4}Assn., J. Low Power Double Data Rate 4 (LPDDR4) Standard. {\em JESD209}. \textbf{4}
\bibitem{hsu2021gptpu}Hsu, K. \& Tseng, H. GPTPU: Accelerating Applications using Edge Tensor Processing Units. {\em ArXiv Preprint ArXiv:2107.05473}. (2021)
\bibitem{kool2018attention}Kool, W., Van Hoof, H. \& Welling, M. Attention, learn to solve routing problems!. {\em ArXiv Preprint ArXiv:1803.08475}. (2018)
\bibitem{zhang2001efficient}Zhang, L., Madigan, C., Moskewicz, M. \& Malik, S. Efficient Conflict Driven Learning in a Boolean Satisfiability Solver. (IEEE Press,2001)
\bibitem{micheli1994synthesis}Micheli, G. Synthesis and Optimization of Digital Circuits. (McGraw-Hill Higher Education,1994)
\bibitem{zhao2015area}Zhao, R., Tan, M., Dai, S. \& Zhang, Z. Area-Efficient Pipelining for FPGA-Targeted High-Level Synthesis. (ACM,2015)
\bibitem{dai2014flushing}Dai, S., Tan, M., Hao, K. \& Zhang, Z. Flushing-Enabled Loop Pipelining for High-Level Synthesis. (ACM,2014)
\bibitem{dai2017dynamic}Dai, S., Zhao, R., Liu, G., Srinath, S., Gupta, U., Batten, C. \& Zhang, Z. Dynamic Hazard Resolution for Pipelining Irregular Loops in High-Level Synthesis. (ACM,2017)
\bibitem{liu2017architecture}Liu, G., Tan, M., Dai, S., Zhao, R. \& Zhang, Z. Architecture and Synthesis for Area-Efficient Pipelining of Irregular Loop Nests. (IEEE,2017)
\bibitem{tan2015elasticflow}Tan, M., Liu, G., Zhao, R., Dai, S. \& Zhang, Z. ElasticFlow: A Complexity-Effective Approach for Pipelining Irregular Loop Nests. (IEEE,2015)
\bibitem{tan2014multithreaded}Tan, M., Liu, B., Dai, S. \& Zhang, Z. Multithreaded Pipeline Synthesis for Data-Parallel Kernels. (IEEE Press,2014)
\bibitem{tan2015mapping}Tan, M., Dai, S., Gupta, U. \& Zhang, Z. Mapping-Aware Constrained Scheduling for LUT-Based FPGAs. (ACM,2015)
\bibitem{ajayi2017celerity}Al, T. Celerity: An Open-Source RISC-V Tiered Accelerator Fabric.  (2017)
\bibitem{ajayi2017experiences}Ajayi, T., Al-Hawaj, K., Amarnath, A., Dai, S., Davidson, S., Gao, P., Liu, G., Rao, A., Rovinski, A., Sun, N., Torng, C., Vega, L., Veluri, B., Xie, S., Zhao, C., Zhao, R., Batten, C., Dreslinski, R., Gupta, R., Taylor, M. \& Zhang, Z. Experiences Using the RISC-V Ecosystem to Design an Accelerator-Centric SoC in TSMC 16nm. {\em First Workshop On Computer Architecture Research With RISC-V (CARRV)}. (2017)
\bibitem{srivastava2017accelerating}Srivastava, N., Dai, S., Manohar, R. \& Zhang, Z. Accelerating Face Detection on Programmable SoC Using C-Based Synthesis.  (2017)
\bibitem{zhou2018rosetta}Zhou, Y., Gupta, U., Dai, S., Zhao, R., Srivastava, N., Jin, H., Featherston, J., Lai, Y., Liu, G., Velasquez, G., Wang, W. \& Zhang, Z. Rosetta: A Realistic Benchmark Suite for Software Programmable FPGAs.  (2018)
\bibitem{liu2016high}Liu, X., Chen, Y., Nguyen, T., Gurumani, S., Rupnow, K. \& Chen, D. High Level Synthesis of Complex Applications: An H.264 Video Decoder. (ACM,2016)
\bibitem{jiang2008scheduling}Jiang, W., Zhang, Z., Potkonjak, M. \& Cong, J. Scheduling with Integer Time Budgeting for Low-Power Optimization. (IEEE Computer Society Press,2008)
\bibitem{dai2017enabling}Dai, S., Liu, G., Zhao, R. \& Zhang, Z. Enabling Adaptive Loop Pipelining in High-Level Synthesis. {\em Asilomar Conf. On Signals, Systems, And Computers}. (2017)
\bibitem{josipovic2017fromc}Josipovic, L., Brisk, P. \& Ienne, P. From C to Elastic Circuits. {\em Asilomar Conf. On Signals, Systems, And Computers}. (2017)
\bibitem{zheng2014fast}Zheng, H., Gurumani, S., Rupnow, K. \& Chen, D. Fast and Effective Placement and Routing Directed High-Level Synthesis for FPGAs. (ACM,2014)
\bibitem{zhang2015high}Zhang, Z., Chen, D., Dai, S. \& Campbell, K. High-Level Synthesis for Low-Power Design. {\em IPSJ Transactions On System LSI Design Methodology (T-SLDM)}. \textbf{8} pp. 12-25 (2015)
\bibitem{cong2010behavior}Cong, J., Liu, B., Majumdar, R. \& Zhang, Z. Behavior-Level Observability Analysis for Operation Gating in Low-Power Behavioral Synthesis. (ACM,2010)
\bibitem{zhang2017high}Zhang, X., Liu, X., Ramachandran, A., Zhuge, C., Tang, S., Ouyang, P., Cheng, Z., Rupnow, K. \& Chen, D. High-Performance Video Content Recognition with Long-Term Recurrent Convolutional Network for FPGA. (IEEE,2017)
\bibitem{zhao2017accelerating}Zhao, R., Song, W., Zhang, W., Xing, T., Lin, J., Srivastava, M., Gupta, R. \& Zhang, Z. Accelerating Binarized Convolutional Neural Networks with Software-Programmable FPGAs. {\em FPGA}. pp. 15-24 (2017)
\bibitem{liang2012high}Liang, Y., Rupnow, K., Li, Y., Min, D., Do, M. \& Chen, D. High-Level Synthesis: Productivity, Performance, and Software Constraints. {\em Journal Of Electrical And Computer Engineering}. \textbf{2012} pp. 1 (2012)
\bibitem{liu2015offline}Liu, J., Bayliss, S. \& Constantinides, G. Offline Synthesis of Online Dependence Testing: Parametric Loop Pipelining for HLS. (IEEE,2015)
\bibitem{alle2013runtime}Alle, M., Morvan, A. \& Derrien, S. Runtime Dependency Analysis for Loop Pipelining in High-Level Synthesis. (ACM,2013)
\bibitem{rau1996iterative}Rau, B. Iterative Modulo Scheduling. {\em International Journal Of Parallel Programming}. \textbf{24}, 3-64 (1996)
\bibitem{canis2014modulo}Canis, A., Brown, S. \& Anderson, J. Modulo SDC Scheduling with Recurrence Minimization in High-Level Synthesis. (IEEE,2014)
\bibitem{zhang2013sdc}Zhang, Z. \& Liu, B. SDC-Based Modulo Scheduling for Pipeline Synthesis. (IEEE Press,2013)
\bibitem{hara2008chstone}Hara, Y., Tomiyama, H., Honda, S., Takada, H. \& Ishii, K. CHStone: A Benchmark Program Suite for Practical C-Based High-Level Synthesis. (IEEE,2008)
\bibitem{marques2008practical}Marques-Silva, J. Practical Applications of Boolean Satisfiability. {\em Int'l Workshop On Discrete Event Systems (WODES)}. pp. 74-80 (2008)
\bibitem{stallman1999using}Stallman, R. Using and Porting the GNU Compiler Collection. {\em Free Software Foundation}. \textbf{86} (1999)
\bibitem{czajkowski2012opencl}Czajkowski, T., Neto, D., Kinsner, M., Aydonat, U., Wong, J., Denisenko, D., Yiannacouras, P., Freeman, J., Singh, D. \& Brown, S. OpenCL for FPGAs: Prototyping a Compiler. {\em Int'l Conf. On Engineering Of Reconfigurable Systems And Algorithms (ERSA)}. pp. 1 (2012)
\bibitem{nieuwenhuis2012sat}Nieuwenhuis, R. SAT and SMT are Still Resolution: Questions and Challenges. {\em Automated Reasoning}. pp. 10-13 (2012)
\bibitem{de2008z3}De Moura, L. \& Bjørner, N. Z3: An Efficient SMT Solver. {\em Tools And Algorithms For The Construction And Analysis Of Systems}. pp. 337-340 (2008)
\bibitem{dutertre2014yices}Dutertre, B. Yices 2.2. {\em Int'l Conf. On Computer Aided Verification (CAV)}. pp. 737-744 (2014)
\bibitem{barrett2011cvc4}Barrett, C., Conway, C., Deters, M., Hadarean, L., Jovanović, D., King, T., Reynolds, A. \& Tinelli, C. CVC4. {\em Int'l Conf. On Computer Aided Verification (CAV)}. pp. 171-177 (2011)
\bibitem{chen2013branch}Chen, M., Huang, S., Pu, G. \& Mishra, P. Branch-and-Bound Style Resource Constrained Scheduling using Efficient Structure-Aware Pruning. {\em IEEE Computer Society Annual Symposium On VLSI (ISVLSI)}. pp. 224-229 (2013)
\bibitem{yu2010place}Yu, C., Wu, Y. \& Wang, S. An In-Place Search Algorithm for the Resource Constrained Scheduling Problem during High-Level Synthesis. (ACM,2010)
\bibitem{wang2005deciding}Wang, C., Ivančić, F., Ganai, M. \& Gupta, A. Deciding Separation Logic Formulae by SAT and Incremental Negative Cycle Elimination. {\em Logic For Programming, Artificial Intelligence, And Reasoning}. pp. 322-336 (2005)
\bibitem{cotton2005satisfiability}Cotton, S., Podelski, A. \& Finkbeiner, B. Satisfiability Checking with Difference Constraints. {\em Int'l Max Planck Research School For Computer Science, Saarbrüceken,Germany}. (2005)
\bibitem{narasimhan2001fast}Narasimhan, M. \& Ramanujam, J. A Fast Approach to Computing Exact Solutions to the Resource-Constrained Scheduling Problem. (ACM,2001)
\bibitem{cbc2005}Forrest, J. CBC User Guide. {\em IBM Research}. \textbf{46}, 157 (2005)
\bibitem{cplex2009v126}CPLEX, I. V12.6: User`s Manual for CPLEX. {\em International Business Machines Corporation}. \textbf{46}, 157 (2015)
\bibitem{biere2013lingeling}Biere, A. Lingeling, Plingeling and Treengeling Entering the SAT Competition 2013. {\em SAT Competition}. \textbf{2013} (2013)
\bibitem{LaAd04:LLVM}Lattner, C. \& Adve, V. LLVM: a Compilation Framework for Lifelong Program Analysis & Transformation.  (2004,3)
\bibitem{chinneck1991locating}Chinneck, J. \& Dravnieks, E. Locating Minimal Infeasible Constraint Sets in Linear Programs. {\em ORSA Journal On Computing}. \textbf{3}, 157-168 (1991)
\bibitem{rim1994lower}Rim, M. \& Jain, R. Lower-bound Performance Estimation for the High-Level Synthesis Scheduling Problem. (IEEE,1994)
\bibitem{ramalingam1999solving}Ramalingam, G., Song, J., Joskowicz, L. \& Miller, R. Solving Systems of Difference Constraints Incrementally. {\em Algorithmica}. \textbf{23}, 261-275 (1999)
\bibitem{van1981irreducibly}Van Loon, J. Irreducibly Inconsistent Systems of Linear Inequalities. {\em European Journal Of Operational Research}. \textbf{8}, 283-288 (1981)
\bibitem{pratt1977two}Pratt, V. Two Easy Theories whose Combination is Hard. (Massachusetts Institute of Technology,1977)
\bibitem{horbach2010boolean}Horbach, A. A Boolean Satisfiability Approach to the Resource-Constrained Project Scheduling Problem. {\em Annals Of Operations Research}. \textbf{181}, 89-107 (2010)
\bibitem{malik2009boolean}Malik, S. \& Zhang, L. Boolean Satisfiability from Theoretical Hardness to Practical Success. {\em Communications Of The ACM}. \textbf{52}, 76-82 (2009)
\bibitem{davis1962machine}Davis, M., Logemann, G. \& Loveland, D. A Machine Program for Theorem-Proving. {\em Communications Of The ACM}. \textbf{5}, 394-397 (1962)
\bibitem{de2011satisfiability}De Moura, L. \& Bjørner, N. Satisfiability Modulo Theories: Introduction and Applications. {\em Communications Of The ACM}. \textbf{54}, 69-77 (2011)
\bibitem{CoZh06:sdc}Cong, J. \& Zhang, Z. An Efficient and Versatile Scheduling Algorithm Based on SDC Formulation.  (2006)
\bibitem{parker1986maha}Parker, A., Pizarro, J. \& Mlinar, M. MAHA: A Program for Datapath Synthesis. (IEEE Press,1986)
\bibitem{canis2011legup}Al., A. LegUp: High-Level Synthesis for FPGA-Based Processor/Accelerator Systems.  (2011)
\bibitem{CoLi11:autoesl}Cong, J., Liu, B., Neuendorffer, S., Noguera, J., Vissers, K. \& Zhang, Z. High-Level Synthesis for FPGAs: From Prototyping to Deployment.  (2011)
\bibitem{ratner2019sysml}Ratner, A., Alistarh, D., Alonso, G., Bailis, P., Bird, S., Carlini, N., Catanzaro, B., Chung, E., Dally, B., Dean, J. \& Others SysML: The New Frontier of Machine Learning Systems. {\em ArXiv Preprint ArXiv:1904.03257}. (2019)
\bibitem{paulin1989force}Paulin, P. \& Knight, J. Force-directed scheduling for the behavioral synthesis of ASICs. {\em IEEE Transactions On Computer-Aided Design Of Integrated Circuits And Systems}. \textbf{8}, 661-679 (1989)
\bibitem{yang1993list}Yang, T. \& Gerasoulis, A. List scheduling with and without communication delays. {\em Parallel Computing}. \textbf{19}, 1321-1344 (1993)
\bibitem{ahn2020ordering}Ahn, B., Lee, J., Lin, J., Cheng, H., Hou, J. \& Esmaeilzadeh, H. Ordering chaos: Memory-aware scheduling of irregularly wired neural networks for edge devices. {\em ArXiv Preprint ArXiv:2003.02369}. (2020)
\bibitem{leiserson1991retiming}Leiserson, C. \& Saxe, J. Retiming synchronous circuitry. {\em Algorithmica}. \textbf{6}, 5-35 (1991)

\end{thebibliography}

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

